Unsupervised representation learning with recognition-parametrised probabilistic models

We introduce a new approach to probabilistic unsupervised learning based on the recognition-parametrised model (RPM): a normalised semi-parametric hypothesis class for joint distributions over observed and latent variables. Under the key assumption that observations are conditionally independent given latents, the RPM combines parametric prior and observation-conditioned latent distributions with non-parametric observation marginals. This approach leads to a flexible learnt recognition model capturing latent dependence between observations, without the need for an explicit, parametric generative model. The RPM admits exact maximum-likelihood learning for discrete latents, even for powerful neural-network-based recognition. We develop effective approximations applicable in the continuous-latent case. Experiments demonstrate the effectiveness of the RPM on high-dimensional data, learning image classification from weak indirect supervision; direct image-level latent Dirichlet allocation; and recognition-parametrised Gaussian process factor analysis (RP-GPFA) applied to multi-factorial spatiotemporal datasets. The RPM provides a powerful framework to discover meaningful latent structure underlying observational data, a function critical to both animal and artificial intelligence.

==> graphical_models/generic.tex <==
\definegmnode{x1}  (-2,0) {graphmod obs, node var={\x_1}}
\definegmnode{x2}  (0,0) {graphmod obs, node var={\x_2}}
\definegmnode{x3}  (2,0) {graphmod obs, node var={\x_3}}
\definegmnode{latent} (0,2) {graphmod lat, node var={\setZ}}


\definegmdefaultnodes{x1, x2,x3, latent} % ,wconc}

\definegmgraph[dag][1][]{\defaultnodes[#1]
  \dedges[#1]{{latent}{x1},{latent}{x2},{latent}{x3}}
}

\definegmgraph[factor][1][]{\defaultnodes[#1]

  \factor[#1,right=1\gmu,label=0:$\fz$]{latent}

  \factor[#1,label=180:$\fxz_1$]{{x1},{latent}}
  \factor[#1,label={[inner sep=-2pt]below right:$\fxz_2$}]{{x2},{latent}}
  \factor[#1,label=0:$\fxz_3$]{{x3},{latent}}

  \factor[below=1\gmu,label=left:$\fx_1$]{x1}
  \factor[below=1\gmu,label=left:$\fx_2$]{x2}
  \factor[below=1\gmu,label=left:$\fx_3$]{x3}

  %% \factor[below=1\gmu,label=-90:{$\fx_1 \to \pxempj({x}_1)$}]{x1}
  %% \factor[below=1\gmu,label=-90:$\pxempj(x_2)$]{x2}
  %% \factor[below=1\gmu,label=-90:$\pxempj(x_3)$]{x3}
}

\definegmgraph[factor.leftlabels][1][]{\defaultnodes[#1]

  \factor[#1,left=1\gmu,label={[label distance=3mm]180:$\fz$}]{latent}

  \factor[#1,label={[label distance=2.2mm]left:$\fxz_j$}]{{x1},{latent}}
  \factor[#1]{{x2},{latent}}
  \factor[#1]{{x3},{latent}}

  \factor[below=1\gmu,label=left:$\fx_j$]{x1}
  \factor[below=1\gmu]{x2}
  \factor[below=1\gmu]{x3}

  %% \factor[below=1\gmu,label=-90:{$\fx_1 \to \pxempj({x}_1)$}]{x1}
  %% \factor[below=1\gmu,label=-90:$\pxempj(x_2)$]{x2}
  %% \factor[below=1\gmu,label=-90:$\pxempj(x_3)$]{x3}
}


\definegmgraph[rpm][1][]{\defaultnodes[#1]

%   \factor[#1,right=1\gmu]{latent}

%   \node at (2.5,2) [right,inner sep=0pt] {$\fz \to \pthetaz(\setZ)$};

  \factor[#1]{{x1},{latent}}
  \factor[#1]{{x2},{latent}}
  \factor[#1]{{x3},{latent}}

  % \node at (2.5,1) [right,inner sep=0pt] {$\fxz_j \to
  %       \frac{\pthetazxj[j](\setZ| \x_j)}
  %            {\angles{\pthetazxj[j](\setZ
  %       | \x_j)}_{\makebox(0,0)[l]{$\scriptscriptstyle \pxempj$}}}
  %       $};


  \factor[below=1\gmu]{x1}
  \factor[below=1\gmu]{x2}
  \factor[below=1\gmu]{x3}

  % \node at (2.5,-1.2) [right,inner sep=0pt] {$\fx_j \to \pxempj(\x_j)$};


  %% \factor[below=1\gmu,label=-90:{$\fx_1 \to \pxempj({x}_1)$}]{x1}
  %% \factor[below=1\gmu,label=-90:$\pxempj(x_2)$]{x2}
  %% \factor[below=1\gmu,label=-90:$\pxempj(x_3)$]{x3}
}

\definegmgraph[rpm_factors][1][]{\defaultnodes[#1]

  \factor[#1,right=1\gmu]{latent}

  \node at (2.5,2) [right,inner sep=0pt] {$\fz \to \pthetaz(\setZ)$};

  \factor[#1]{{x1},{latent}}
  \factor[#1]{{x2},{latent}}
  \factor[#1]{{x3},{latent}}

  \node at (2.3,0.9) [right,inner sep=0pt] {$\fxz_j \to
        \frac{\pthetazxj[j](\setZ| \x_j)}
             {\angles{\pthetazxj[j](\setZ
        | \x_j)}_{\makebox(0,0)[l]{$\scriptscriptstyle \pxempj$}}}
        $};


  \factor[below=1\gmu]{x1}
  \factor[below=1\gmu]{x2}
  \factor[below=1\gmu]{x3}

  \node at (2.5,-1.2) [right,inner sep=0pt] {$\fx_j \to \pxempj(\x_j)$};
}



==> graphical_models/gpfa_gen.tex <==
\definegmnode{x11}  (-2,+0) {graphmod obs, node var={\x_{11}}}
\definegmnode{x12}  (0,+0) {graphmod obs, node var={\x_{12}}}
\definegmnode{x13}  (2,+0) {graphmod ghost, node var={\dots}}
\definegmnode{x1T}  (4,+0) {graphmod obs, node var={\x_{1T}}}

\definegmnode{x21}  (-2,-1) {graphmod ghost, node var={\vdots}}
\definegmnode{x22}  (+0,-1) {graphmod ghost, node var={\vdots}}
\definegmnode{x23}  (+2,-1) {graphmod ghost, node var={}}
\definegmnode{x2T}  (+4,-1) {graphmod ghost, node var={\vdots}}

\definegmnode{xJ1}  (-2,-2) {graphmod obs, node var={\x_{J1}}}
\definegmnode{xJ2}  (+0,-2) {graphmod obs, node var={\x_{J2}}}
\definegmnode{xJ3}  (+2,-2) {graphmod ghost, node var={\dots}}
\definegmnode{xJT}  (+4,-2) {graphmod obs, node var={\x_{JT}}}

\definegmnode{latent} (0,2) {graphmod lat, node var={z}}

\definegmnode{z1} (-2,2) {graphmod lat, node var={\z_1}}
\definegmnode{z2} (+0,2) {graphmod lat, node var={\z_2}}
\definegmnode{z3} (+2,2) {graphmod ghost, node var={\dots}}
\definegmnode{zT} (+4,2) {graphmod lat, node var={\z_T}}


%\definegmdefaultnodes{x1, x2,x3, latent} % ,wconc}

\definegmdefaultnodes{
x11, x12, x13, x1T, 
x21, x22, x23, x2T, 
xJ1, xJ2, xJ3, xJT, 
z1, z2, z3, zT} % ,wconc}

\definegmgraph[gen][1][]{\defaultnodes[#1]
  \dedges[#1]{{z1}{z2},{z2}{z3}, {z3}{zT}} 
  
  
  \draw[black, thick]  (-2,+1.5) edge[out=-120, in=120, -to] (-2-0.1,+0.5);
  \draw[black, thick]  (-2,+1.5) edge[out=-140, in=140, -to] (-2-0.1,-1.5);
  \draw[black, thick]  (+0,+1.5) edge[out=-120, in=120, -to] (+0-0.1,+0.5);
  \draw[black, thick]  (+0,+1.5) edge[out=-140, in=140, -to] (+0-0.1,-1.5);
  \draw[black, thick]  (+4,+1.5) edge[out=-120, in=120, -to] (+4-0.1,+0.5);
  \draw[black, thick]  (+4,+1.5) edge[out=-140, in=140, -to] (+4-0.1,-1.5);
  
}




%\definegmgraph[rpm][1][]{\defaultnodes[#1]
%  \factor[#1]{{x1},{latent}}
%  \factor[#1]{{x2},{latent}}
%  \factor[#1]{{x3},{latent}} 
  
%  \factor[below=1\gmu,label=-90:$p_0(x_1)$]{x1}
%  \factor[below=1\gmu,label=-90:$p_0(x_2)$]{x2}
%  \factor[below=1\gmu,label=-90:$p_0(x_3)$]{x3}
%}


==> graphical_models/gpfa_rpm.tex <==

\definegmnode{latent} (0.0,+0.2) {graphmod lat, node var={\z_{t}\nn}}
\definegmnode{prior}  (-3,0.2) {graphmod lat, node var={\kappa}}
\definegmnode{nnet}   (-3.0,-1.5) {graphmod lat, node var={\theta_{j}}}
\definegmnode{obsx}   (0.0,-3.2) {graphmod obs, node var={\x_{tj}\nn}}
\definegmnode{ip}     (+2.5,0.2) {graphmod lat, node var={\scriptstyle \setU\nn}}

\definegmnode{ghost1} (-0.5,-3.2) {graphmod ghost, node var={}}
\definegmnode{ghost2} (+0.2,-3.8) {graphmod ghost, node var={}}
\definegmnode{ghost3} (0.0,-4.2) {graphmod ghost, node var={}}


\gmsetstyle[plate font={\scriptscriptstyle}]{plate label}
\gmsetstyle[plate label={\text{factor } j=1\dots J}]{plate nnetobsxghost2 label}
\gmsetstyle[plate label={\text{time } t=1\dots T}]{plate latentobsxghost1 label}

\gmsetstyle[inner xsep=0.3\gmu]{plate nnetobsxlatent}
\gmsetstyle[plate label={\text{observation } n=1\dots N}]
           {plate latentobsxghost1ipghost3 label}


\definegmdefaultnodes{ prior, latent, obsx, nnet, ip, ghost1, ghost2, ghost3} 


\definegmgraph[rpm][1][]{\defaultnodes[#1]
  %\gmaddstyle[#1]{plate wordtopic label, plate wordtopictdir label,
  %  plate wdir label} % plate labels need special option handling
  \factor[right=1.5\gmu,label=0:$\scriptstyle p_{0, jt}$]{obsx}
  
  \plate[#1]{nnet,obsx,ghost2}
  \plate[#1]{latent,obsx,ghost1}
  \plate[#1]{plate latentobsxghost1,ip,ghost3}
  \dedges[#1]{{prior}{latent}, {ip}{latent}}
  \factor[#1]{latent,nnet,obsx}
  
  
  

}



==> graphical_models/hmm.tex <==
\definegmnode{x11}  (-2,+0) {graphmod obs, node var={\x_{1}}}
\definegmnode{x12}  (0,+0) {graphmod obs, node var={\x_{2}}}
\definegmnode{x13}  (2,+0) {graphmod ghost, node var={\dots}}
\definegmnode{x1T}  (4,+0) {graphmod obs, node var={\x_{T}}}

\definegmnode{z1} (-2,2) {graphmod lat, node var={\z_1}}
\definegmnode{z2} (+0,2) {graphmod lat, node var={\z_2}}
\definegmnode{z3} (+2,2) {graphmod ghost, node var={\dots}}
\definegmnode{zT} (+4,2) {graphmod lat, node var={\z_T}}


%\definegmdefaultnodes{x1, x2,x3, latent} % ,wconc}

\definegmdefaultnodes{
x11, x12, x13, x1T, 
z1, z2, z3, zT} % ,wconc}

\definegmgraph[gen][1][]{\defaultnodes[#1]
  \dedges[#1]{{z1}{z2},{z2}{z3}, {z3}{zT}} 
  \dedges[#1]{{z1}{x11}, {z2}{x12}, {zT}{x1T}} 
  
}




%\definegmgraph[rpm][1][]{\defaultnodes[#1]
%  \factor[#1]{{x1},{latent}}
%  \factor[#1]{{x2},{latent}}
%  \factor[#1]{{x3},{latent}} 
  
%  \factor[below=1\gmu,label=-90:$p_0(x_1)$]{x1}
%  \factor[below=1\gmu,label=-90:$p_0(x_2)$]{x2}
%  \factor[below=1\gmu,label=-90:$p_0(x_3)$]{x3}
%}


==> graphical_models/lda.tex <==
\definegmnode{word}  (0,0) {graphmod obs, node var={\x_{j}\nn}}
\definegmnode{topic} (0,2) {graphmod lat, node var={\z_{j}\nn}}
\definegmnode{tdir}  (0,4) {graphmod lat, node var={\omega\nn}}
\definegmnode{wdir}  (2,1) {graphmod lat, node var={\theta}}
\definegmnode{tconc} (0,6) {graphmod lat, node var={\alpha}}
\definegmnode{wconc} (3,4) {graphmod lat, node var={\beta}}

\gmsetstyle[plate font={\scriptscriptstyle}]{plate label}
\gmsetstyle[plate label={\text{} j=1\dots J}]{plate wordtopic label}
\gmsetstyle[inner xsep=0.3\gmu]{plate wordtopictdir}
\gmsetstyle[plate label={\text{image } n=1\dots N}]
           {plate wordtopictdir label}
\gmsetstyle[plate label={\text{topic } k=1\dots K}]
           {plate wdir label} 

\definegmdefaultnodes{word,topic,tdir,wdir,tconc} % ,wconc}

\definegmgraph[1][]{\defaultnodes[#1]
  \gmaddstyle[#1]{plate wordtopic label, plate wordtopictdir label,
    plate wdir label} % plate labels need special option handling
  \plate[#1]{word,topic}%
  \plate[#1]{plate wordtopic,tdir}%
%  \plate[#1]{wdir}%
  \dedges[#1]{{topic}{word},{wdir}{word},{tdir}{topic},{tconc}{tdir}} % ,{wconc}{wdir}}
}


\definegmgraph[rpm][1][]{\defaultnodes[#1]
  \gmaddstyle[#1]{plate wordtopic label, plate wordtopictdir label,
    plate wdir label} % plate labels need special option handling
  \plate[#1]{word,topic}%
  \plate[#1]{plate wordtopic,tdir}%
%  \plate[#1]{wdir}%
  \dedges[#1]{{tdir}{topic},{tconc}{tdir}} % {topic}{word},{wdir}{word},,{wconc}{wdir}}
  \factor[#1]{word,topic,wdir}
  \factor[left=1.5\gmu, label=180:$p_0$, #1]{word}
}



==> graphical_models/peer_supervision_gen.tex <==
\definegmnode{x1}(+1,+1.5) {graphmod obs, node var={\x_{1}}}
\definegmnode{x2}(+1,-1.5) {graphmod obs, node var={\x_{2}}}
\definegmnode{z} (-1,+0) {graphmod lat, node var={\z}}
\definegmnode{theta} (+2,+0) {graphmod lat, node var={\theta}}



%\definegmdefaultnodes{x1, x2,x3, latent} % ,wconc}

\definegmdefaultnodes{x1, x2, z}


\definegmgraph[genpeer][1][]{\defaultnodes[#1]
  \dedges[#1]{{z}{x1},{z}{x2}}
  }
  
 



==> graphical_models/peer_supervision_rpm.tex <==
\definegmnode{x1}(+1,+1.5) {graphmod obs, node var={\x_{j} \nn}}
\definegmnode{z} (-1,+1.5) {graphmod lat, node var={\z \nn}}
\definegmnode{theta} (+0,-1) {graphmod lat, node var={\theta}}

\definegmnode{g1}(+1.2,+1.7) {graphmod ghost, node var={}}
\definegmnode{g2}(+1.2,+1.0) {graphmod ghost, node var={}}


%\definegmdefaultnodes{x1, x2,x3, latent} % ,wconc}

\definegmdefaultnodes{x1, theta, z, g1, g2}


\gmsetstyle[plate font={\scriptscriptstyle}]{plate label}
\gmsetstyle[plate label={\text{} n=1\dots N}]{plate zx1g2g1 label}
\gmsetstyle[plate label={\text{ } j=1,2}]{plate x1 label}


\definegmgraph[rpmpeer][1][]{\defaultnodes[#1]
  \factor[#1]{z,x1,theta}
  \plate[#1]{z,x1,g2,g1}
  \plate[#1]{x1}
  
  \factor[above=1.5\gmu,label=0:$\scriptstyle p_{0, j}$]{x1}
  }
  
 



==> graphical_models/peer_supervision_rpm2.tex <==
\definegmnode{x1}(+1,+1.5) {graphmod obs, node var={\x_{1} \nn}}
\definegmnode{x2}(+1,-1.5) {graphmod obs, node var={\x_{2} \nn}}
\definegmnode{z} (-1,0)  {graphmod lat, node var={\z \nn}}

\definegmnode{theta} (2.5,0)  {graphmod lat, node var={\theta}}



%\definegmdefaultnodes{x1, x2,x3, latent} % ,wconc}

\definegmdefaultnodes{x1, x2, theta, z}

\gmsetstyle[plate font={\scriptscriptstyle}]{plate label}
\gmsetstyle[plate label at=south west, plate label={\text{} n=1\dots N}]{plate zx1x2 label}
\gmsetstyle[plate label={\text{ } j=1,2}]{plate x1 label}


\definegmgraph[rpmpeer][1][]{\defaultnodes[#1]
  \factor[#1]{z,x1}
  \factor[#1]{z,x2}
  \edges{factor zx1--theta}
  \edges{factor zx2--theta}
  \factor[right=1\gmu,label=0:$\scriptstyle p_{0}$]{x1}
  \factor[right=1\gmu,label=0:$\scriptstyle p_{0}$]{x2}
  \plate[#1,inner sep=0.1\gmu]{z,x1,x2}
}
  
 



==> m.macros.tex <==
\makeatletter

\newcommand{\define}[1]{{\bf #1}}
\newcommand{\figpanel}[1]{\textsf{#1}}
\newcommand{\todo}[1]{}
%\newcommand{\todo}[1]{[\textit{TODO: #1}]}

% some abbreviations

\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}

\newcommand{\intinf}{\int_{-\infty}^{+\infty}}

% reference styles
\newcommand{\chpref}[1]{chapter~\ref{chp:#1}}
\newcommand{\Chpref}[1]{Chapter~\ref{chp:#1}}
\newcommand{\secref}[1]{section~\ref{sec:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[2]{figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\Figref}[2]{Figure~\ref{fig:#1}\figpanel{#2}}
\newcommand{\eqnref}[1]{(\ref{eqn:#1})}
\newcommand{\Eqnref}[1]{Equation (\ref{eqn:#1})}

% set horizontal margins to center text (using current paperwidth & textwidth)
\def\equalmargins{
	\setlength{\oddsidemargin}{\paperwidth}
	\addtolength{\oddsidemargin}{-\textwidth}
	\setlength{\oddsidemargin}{0.5 \oddsidemargin}
	\addtolength{\oddsidemargin}{-1in}
	\setlength{\evensidemargin}{\oddsidemargin}
}


% force equation numbers
\newenvironment{eqnforce}[1]{%
\let\savetheequation=\theequation% save the old equation number defn
\renewcommand{\theequation}{#1}%   set the equation string
\begin{equation}%		   start a normal equation env
}{%
\end{equation}%			   end it
\let\theequation=\savetheequation% restore the old defn
\addtocounter{equation}{-1}%       restore the counter which was incremented
}

% abbreviate \nonumber\\
\newcommand{\nn}{\nonumber\\}

% make text in super/subscripts the right size
\newcommand\mathbox[1]{\mathchoice{\mbox{#1}}{\mbox{#1}}%
{\mbox{\scriptsize{#1}}}{\mbox{\tiny{#1}}}}


% et al.
\newcommand{\etal}{\textit{et al$.$}}

% move the control point of the argument to the bottom of the box ...
\def\alignbottom#1{%
  \setbox0=\hbox{#1}%
  \raise\dp0\box0%
}
% ... or to the top ...
\newcommand{\aligntop}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=-\ht0%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}
% ... or to the middle.

\newcommand{\alignmiddle}[2][0pt]{%
  \setbox0=\hbox{#2}%
  \dimen0=\dp0%
  \advance\dimen0 by -\ht0%
  \divide\dimen0 by 2%
  \advance\dimen0 by #1%
  \raise\dimen0\box0%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TikZ tricks

\RequirePackage{tikz}

%% Create inline node: shorthand for \tikz[baseline,OPT1]{\node [OPT2] {ARG}}
%% some uses:
%% \tikznode[base]{foo}   
%% \tikznode[middle]{foo} 
%% \tikznode[below]{foo}
%% \tikznode[below=-1ex]{foo}
%% \tikznode[draw=red]{foo}       % tight red frame
%% \tikznode[framed=blue]{foo}    % adds some space (can be adjusted w/ inner sep
\newcommand\tikznode[1][]{%
  \@ifnextchar[{\m@tikznode[#1]}{\m@tikznode[][#1]}}
\def\m@tikznode[#1][#2]#3{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
  \tikz[baseline,#1]{\node [anchor=base,inner sep=0pt, #2] {#3};}%
  \endgroup%
}

%% Option to \path to annotate within a node (eg place text on a figure):
%% \node (fig) {\includegraphics{}};
%% \path[fit to node=fig] (0.1, 1) node {A};
\tikzoption{fit to node}{\tikzset{shift=(#1.south west), x=(#1.south east), y=(#1.north west)}}


%% Option to tikzpicture to set coords based on column/text size
\def\c@@rdx(#1,#2){#1}
\def\c@@rdy(#1,#2){#2}
\tikzset{%
  fit to column/.style={x ={($\c@@rdx#1*(\columnwidth,0)$)},y={($\c@@rdy#1*(0,\textheight)$)}},
  fit to column/.default={(1,1)}
}

%% Create inline node with pin label box pointing to content
%% \tikznodepin[env opts][inline node opts]{inline text}(pos)[pinnode
%% opts][pin edge opts]{pin text}

\tikzstyle{tikznode label node}=[]
\tikzstyle{tikznode label edge}=[->, very thick]
\tikzoption{tikznode label position}{#1\tikznodelabel@setposition#1}
\def\tikznodelabel@setposition(#1){\def\tikznodelabel@position{#1}}
\def\tikznodelabel@position{0, 5ex}

\def\tikznodelabel{%
  \@ifnextchar[{\tikznodelabel@m}{\tikznodelabel@@m[][]}
}
\def\tikznodelabel@m[#1]{%
  \@ifnextchar[{\tikznodelabel@@m[#1]}{\tikznodelabel@@m[][#1]}
}
\def\tikznodelabel@@m[#1][#2]#3{%
  \@ifnextchar({\tikznodelabel@@@m[#1][#2]{#3}}
               {\tikznodelabel@@@m[#1][#2]{#3}(\tikznodelabel@position)}
}
\def\tikznodelabel@@@m[#1][#2]#3(#4){%
  \@ifnextchar[{\tikznodelabel@@@@m[#1][#2]{#3}(#4)}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[][]}
}
\def\tikznodelabel@@@@m[#1][#2]#3(#4)[#5]{%
  \@ifnextchar[{\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5]}
               {\tikznodelabel@@@@@m[#1][#2]{#3}(#4)[#5][]}
}
\def\tikznodelabel@@@@@m[#1][#2]#3(#4)[#5][#6]#7{%
  \begingroup%
  \tikzstyle{descending}=[below=-1.5ex]%
  \tikzstyle{base}=[anchor=base]%
  \tikzstyle{center}=[anchor=center]%
  \tikzstyle{framed}=[inner sep=2pt, draw=##1]%
  \tikzstyle{tight}=[inner sep=0pt]%
  \tikzstyle{smash}=[text height=0pt, text depth=0pt]%
%
  \tikz[baseline,#1]{
    \node (inl) [anchor=base,inner sep=0pt, #2] {#3};
    \useasboundingbox;
    \path (#4) node [tikznode label node, #5] {#7} 
               edge [tikznode label edge, #6] (inl);
   }%
  \endgroup%
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Parse a comma-separated list.  
%
% Latex provides \@for\var=first,second,...,last\do{code} which
% executes {code} many times, each time setting \var to the next item in
% the list 
% 
% This provides a variant \@forlast\var:=a,b,...,z\do{code}{codelast}
% which differs only on the last entry, for which it executes {codelast}.

\long\def\@forlast#1:=#2\do#3#4{%
  \expandafter\def\expandafter\@forlasttmp\expandafter{#2}%
  \ifx\@forlasttmp\@empty%
  \else%
    \expandafter\@forlastloop#2,\@nil,\@nil\@@#1{#3}{#4}%
  \fi%
}

\long\def\@forlastloop#1,#2,#3\@@#4#5#6{%
  \def#4{#1}%
  \ifx #4\@nnil%
    % empty list -- do nothing
  \else%
    \ifx #2\@nil% check if single item
      #6% apply #6 to #1
    \else%
      #5% apply #5 to #1
      \@forlastloop#2,#3\@@#4{#5}{#6}
    \fi%
  \fi%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Grab this page from an image file.  Can be used for a background.
%%   This version works 

%\newcommand\pageimage[1]{%
%  \hspace{-\oddsidemargin}\hspace*{-1in}%
%  \vspace*{-\topmargin}\vspace*{-\headheight}\vspace*{-\headsep}\vspace*{-1in}%
%  \makebox[top,left](0,0)\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio}{#1}
%} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% panel sizes.  

\let\panelwidth\columnwidth
\let\panelheight\textheight


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% image resizing.  width and height give maxima in terms of
%%   columnwidth and textheight respectively.

\def\parsesize[#1,#2]{{#1\panelwidth}{#2\panelheight}}

%% column image is deprecated

\def\mycolumnimage[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}
\newcommand{\columnimage}[2][1,.98]{\mycolumnimage[#1][]{#2}}

\def\mycenterimage[#1,#2][#3]#4{%
  \begin{center}\mycolumnimage[#1,#2][#3]{#4}\end{center}}



\newcommand{\centerimage}[2][1,.98]{\mycenterimage[#1][]{#2}}

\def\myvcenterimage[#1,#2][#3]#4{%
  \vfill\mycenterimage[#1,#2][#3]{#4}\vfill}
\newcommand{\vcenterimage}[2][1,.98]{\myvcenterimage[#1][]{#2}}

\newcommand{\columnline}[2][1]{\hbox to #1\panelwidth{#2}}
\renewcommand{\centerline}[2][1]{\hbox to #1\panelwidth{\hfil #2 \hfil}}


\newcommand{\columnimagestack}[2][1,.98]{%
  \@forlast\n@xtimg:=#2\do%
     {\makebox(0,0)[lb]{\mycolumnimage[#1][]{\n@xtimg}}}%
     {\mycolumnimage[#1][]{\n@xtimg}}%
}

%% so is scaleimage

\def\ScaleImgTwoOpt[#1,#2][#3]#4{%
  \includegraphics[width=#1\panelwidth,height=#2\panelheight,keepaspectratio,#3]%
  {#4}}

\def\ScaleImgOneOpt[#1,#2]{%
  \@ifnextchar[%]
    {\ScaleImgTwoOpt[#1,#2]}%
    {\ScaleImgTwoOpt[#1,#2][]}%
}

\def\scaleimage{%
  \@ifnextchar[%]
    {\ScaleImgOneOpt}%
    {\ScaleImgOneOpt[1,1]}%
}        

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% beamer extensions
\@ifclassloaded{beamer}{

%% Beamer controlled underbrace.  
%% \underbraceon<spec>[prefix]{maintext}{subtext}
%%   - prefix should probably live outside the \alt anyway
\newcommand<>{\underbraceon}[3][]{%
  \alt#4{%
    {#1{\underset{#3}{\underset{\text{\upbracefill}}{#2}}}}
  }{
    {#1{\underset{\phantom{#3}}{\underset{\phantom{\text{\upbracefill}}}{#2}}}}
  }%
}

} % end if beamer



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% pgf extensions

\def\pgfp@nelparsearg[#1,#2]{%
  \def\pgfp@nelwidth{#1\panelwidth}%
  \def\pgfp@nelheight{#2\panelheight}}

\newenvironment{pgfpanel}[1][1,.995]
  {\pgfp@nelparsearg[#1]
   \begin{pgfpicture}{0cm}{0cm}{\pgfp@nelwidth}{\pgfp@nelheight}
      \pgftranslateto{\pgfpoint{0cm}{\pgfp@nelheight}}
      \pgfsetxvec{\pgfpoint{\pgfp@nelwidth}{0cm}}
      \pgfsetyvec{\pgfpoint{0cm}{-\pgfp@nelheight}}}
  {\end{pgfpicture}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% these use pgf to place a box at an arbitrary spot and (second form)
%% draw an arrow to the current position

\newcommand\placebox[4][left,baseline]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfputat{\pgfpoint{#2}{#3}}{\pgfbox[#1]{#4}}
  \end{pgfpicture}%
}

\newcommand\arrowbox[4][{0cm}{0cm}]{%
  \begin{pgfpicture}{0cm}{0cm}{0cm}{0cm}
    \pgfnodebox{text}[virtual]{\pgfpoint{#2}{#3}}{#4}{2pt}{2pt}
    \pgfnodecircle{origin}[virtual]{\pgfpoint#1}{0pt}
    \pgfsetlinewidth{.5mm}
    \pgfsetendarrow{\pgfarrowsingle}
    \pgfnodeconnline{text}{origin}
  \end{pgfpicture}
}




% \def\alignmiddle#1{%
%   \setbox0=\hbox{#1}%
%   \dimen0=\dp0%
%   \advance\dimen0 by -\ht0%
%   \divide\dimen0 by 2%
%   \raise\dimen0\box0%
% }


\makeatother


==> m.symbols.tex <==
\RequirePackage{ifthen}

% use | for math mode
%\catcode`\|=3

% use textmode for a short minus sign
\newcommand{\tminus}{\text{\textendash}}
% equal in expectation
\newcommand{\eqexpect}{\stackrel{\mathcal{E}}{=}}
% conditional independence
\newcommand{\cind}{{\bot\negthickspace\negthickspace\bot}} 
\newcommand{\notcind}{{\smash{\kern0.1em\not\kern-.1em}\cind}}




% Utilities to define pretty functions
\makeatletter

% Functions with resizeable delimiters
%
% \DeclareResizableDelimFunction{macroname}{symbol}{left delim}{right delim}
%
% E.g. \DeclareResizableDelimFunction{foo}{\text{foo}}[]
% defines:
% \foo{x} -> \text{foo} \left[ x \right]
% \foo[\big]{x} -> \text{foo} \big[ x \big]
\def\DeclareResizableDelimFunction#1#2#3#4{
  \expandafter\newcommand\csname#1\endcsname[2][]{%
    #2\lr[##1]#3#4{##2}}}

% \DeclareResizableDelimFunction{macroname}{symbol}{left delim}{right delim}{separator}
%
% E.g. \DeclareResizableDelimFunction{foo}{\text{foo}}[]{,}
% defines:
% \foo{x}{y} -> \text{foo} \left[ x , y\right]
% \foo[\big]{x}{y} -> \text{foo} \big[ x , y \big]
%
% \DeclareResizableDelimFunction{foo}{\text{foo}}[]{\lrmid \|}
% defines:
% \foo{x}{y} -> \text{foo} \left[ x \middle \|  y\right]
% \foo[\big]{x}{y} -> \text{foo} \big[ x \big \|  y \big]
\def\DeclareResizableDelimFunctionOnTwoArgs#1#2#3#4#5{
  \expandafter\newcommand\csname#1\endcsname[3][]{%
    #2\lr[##1]#3#4{##2 #5 ##3}}}

% Optional subscripted functions with resizeable delimiters
%
% \DeclareOptSubscriptedFunction{macroname}{symbol}[default subscr]{left delim}{right delim}
%
% E.g. \DeclareOptSubscriptedFunction{foosq}{\text{foo}^2}[][]
% defines:
% \foosq{x} -> \text{foo}^2 \left[ x \right]
% \foosq[a]{x} -> \text{foo}^2_a \left[ x \right]
% \foosq[a][\big]{x} -> \text{foo}^2_a \big[ x \big]
% \foosq[][\big]{x} -> \text{foo}^2 \big[ x \big]
% \foosq[][][()]{x} -> \text{foo}^2 \left ( x \right )
% Note that _{} would normally add undesirable space that this definition avoids
\def\OptSubscript#1{\ifthenelse{\equal{#1}{}}{}{_{#1}}}
\def\DeclareOptSubscriptFunction#1#2[#3]#4#5{
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar[{\csname#1@\endcsname}{\csname#1@@@\endcsname[#3][][{#4}{#5}]}}
  %
  \expandafter\def\csname#1@\endcsname[##1]{%
    \@ifnextchar[{\csname#1@@\endcsname[##1]}{\csname#1@@@\endcsname[##1][][{#4}{#5}]}}
  %
  \expandafter\def\csname#1@@\endcsname[##1][##2]{%
    \@ifnextchar[{\csname#1@@@\endcsname[##1][##2]}{\csname#1@@@\endcsname[##1][##2][{#4}{#5}]}}
  %
   \expandafter\def\csname#1@@@\endcsname[##1][##2][##3##4]##5{%
%               {\ensuremath{#2\OptSubscript{##1}|##2|##3|##4|##5|}}}
               {\ensuremath{#2\OptSubscript{##1}\lr[##2]{##3}{##4}{##5}}}}
}
\def\DeclareOptSubscriptOptArgFunction#1#2[#3]#4#5{
  \expandafter\def\csname#1\endcsname{%
    \@ifnextchar[{\csname#1@\endcsname}{\csname#1@@@\endcsname[#3][][{#4}{#5}]}}
  %
  \expandafter\def\csname#1@\endcsname[##1]{%
    \@ifnextchar[{\csname#1@@\endcsname[##1]}{\csname#1@@@\endcsname[##1][][{#4}{#5}]}}
  %
  \expandafter\def\csname#1@@\endcsname[##1][##2]{%
    \@ifnextchar[{\csname#1@@@\endcsname[##1][##2]}{\csname#1@@@\endcsname[##1][##2][{#4}{#5}]}}
  %
   \expandafter\def\csname#1@@@\endcsname[##1][##2][##3##4]##5{%
     \ifthenelse{\equal{##5{}}{{}}}% if arg is empty omit delimeters
                {\ensuremath{#2\OptSubscript{##1}}}%
                {\ensuremath{#2\OptSubscript{##1}\lr[##2]{##3}{##4}{##5}}}}
}

\makeatother


% probability distributions
\DeclareOptSubscriptOptArgFunction{pr}{{\bf\sf{P}}}[]()
% \DeclareOptSubscriptFunction{prf}{\bf\sf{P}}[]{}{}

% \newcommand{\pr}[2] {\ensuremath{{\bf\mathsf{P}}_{#1}\left({#2}\right)}}
% \newcommand{\prf}[1] {\ensuremath{{\bf\sf P}_{#1}}}
% \newcommand{\prm}[2]{\ensuremath{{\bf\sf P}\left({#2} ; {#1}\right)}}

% expectations
% \expect{x}        -> \mathbb{E}\left[x\right]
% \expect[a]{x}     -> \mathbb{E}_a\left[x\right]
% \expect[a][\size]{x} -> \mathbb{E}_a \size[ x \size]
\DeclareOptSubscriptFunction{expect}{\mathbb{E}}[][]
\DeclareOptSubscriptFunction{var}{\mathbb{V}}[][]
\DeclareResizableDelimFunction{angles}{}\langle\rangle

% likelihoods
\DeclareOptSubscriptFunction{like}{\mathcal{L}}[]()
\DeclareOptSubscriptFunction{loglike}{\ell}[]()

% info theoretic
\DeclareResizableDelimFunction{entropy}{\textbf{\textsf{H}}}[]
\DeclareResizableDelimFunctionOnTwoArgs{info}{\textbf{\textsf{I}}}[]{\,;}
\def\mutualinfo[#1;#2]{\info{#1}{#2}} % older form
\DeclareResizableDelimFunctionOnTwoArgs{KL}{\textbf{\textsf{KL}}}[]{\lrmid\|}
% \newcommand{\given}{\mid}
\newcommand{\condind}{\perp\!\!\!\perp}

\newcommand{\dist}{\sim}
\newcommand{\distiid}{\stackrel{\mathrm{iid}}{\sim}}

% The normal distribution
\DeclareResizableDelimFunctionOnTwoArgs{normal}{\mathcal{N}}(){,}

% fractions
\newcommand{\half}{\ensuremath{{1\over2}}}
\newcommand{\overN}{\ensuremath{{1\over N}}}
%\newcommand{\tfrac}[2]{\ensuremath{{\textstyle\frac{#1}{#2}}}}
%\newcommand{\dfrac}[2]{\ensuremath{{\frac{\displaystyle #1}{\displaystyle #2}}}}

% whitened quantities
% \newcommand{\white}[1]{\ensuremath{\tilde{#1}}}

% set symbols
\newcommand{\set}[1]{\ensuremath{\mathcal{#1}}}
% explicitly defined in some old versions
% \newcommand{\setV}{\ensuremath{{\cal V}}}
% \newcommand{\setX}{\ensuremath{{\cal X}}}
% \newcommand{\setY}{\ensuremath{{\cal Y}}}
% \newcommand{\setZ}{\ensuremath{{\cal Z}}}
\DeclareResizableDelimFunction{size}{}\vert\vert

% graph stuff
\newcommand{\parent}[1]{\ensuremath{\mathsf{pa}({#1})}}
\newcommand{\child}[2]{\ensuremath{\mathsf{ch}_{#1}({#2})}}
\newcommand{\branch}[2]{\ensuremath{\mathsf{br}_{#1}({#2})}}
\newcommand{\nondes}[1]{\ensuremath{\mathsf{nd}({#1})}}

% matrix stuff
\renewcommand{\vec}[1]{\ensuremath{\mathchoice%
{\mbox{\boldmath$\displaystyle\mathsf{#1}$}}%
{\mbox{\boldmath$\textstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptstyle\mathsf{#1}$}}%
{\mbox{\boldmath$\scriptscriptstyle\mathsf{#1}$}}}}
\newcommand{\mat}[1]{\ensuremath{\mathsf{#1}}}

\newcommand{\coord}[1]{\ensuremath{\vec{e}_{#1}}}
\newcommand{\kron}{\otimes}
\newcommand{\vecop}[1]{\mathop{\mathsf{vec}}\left({#1}\right)}

% transpose/inverse
\newcommand{\tr} {\ensuremath{^{\mathsf{T}}}}
\newcommand{\inv} {\ensuremath{^{-1}}}
\newcommand{\pinv}{\ensuremath{^{\dagger}}}

% vector norm
\DeclareResizableDelimFunction{norm}{}\|\|
\newcommand{\ones}{\vec{\mathsf{1}}}

% determinant, trace, etc
\let\det\undefined % lose std definition
\DeclareResizableDelimFunction{det}{}\vert\vert
\DeclareResizableDelimFunction{trace}{\mathsf{Tr}}[]
\DeclareResizableDelimFunction{diag}{\mathbox{\textsf{diag}}}[]

% derivatives
\newcommand{\grad}{\ensuremath{\nabla}}
\newcommand{\hessian}{\ensuremath{\nabla\nabla}}
\newcommand{\Partial}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\PartialSquare}[2]{\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\PPartial}[2]{\frac{\partial^2 #1}{\partial #2^2}}

%% The following allow constructs like 
%%   \MPartial[3]{f}{x}[2]{y} 
%% for 
%% \frac{\partial^3 f}{\partial x \partial y^2}
\makeatletter
\newcounter{multderiv@ctr}
\newcommand{\MPartial}[2][1]{% 
  \setcounter{multderiv@ctr}{0}% number of denominators read
  \mpartial@next[#1]{#2}{}%      read first denominator
}
\def\mpartial@next[#1]#2#3{% [total order]{numerator}{denoms so far}
  \ifthenelse{\value{multderiv@ctr}<#1}{% more to read
    \@ifnextchar[{\mpartial@next@order[#1]{#2}{#3}}%    this denom has an order
                 {\mpartial@next@order[#1]{#2}{#3}[1]}% default order of 1
                %]
  }{% done with denoms
    \frac{\partial\ifthenelse{#1>1}{^{#1}}{}{#2}}{#3}% render partial
  }%
}
\def\mpartial@next@order[#1]#2#3[#4]#5{%[total ord]{num}{denoms}[this order]{this denom}
  \addtocounter{multderiv@ctr}{#4}% read another denom
  % add this denom to 
  \mpartial@next[#1]{#2}{#3 \partial#5\ifthenelse{#4>1}{^{#4}}{}}}
\makeatother  

\newcommand{\Deriv}[2]{\frac{d#1}{d#2}}
\newcommand{\DDeriv}[2]{\frac{d^2{#1}}{{d#2}^2}}
\newcommand{\varderiv}[2]{\frac{\delta #1}{\delta #2}}

% integral signs -- fix spacing if no limits
\newcommand{\intdx}[1][dx]{%
  % best spacing depends on mathmode
  \mathchoice%
    {\int\!\!#1\,}% display
    {\int\!#1\,}% inline
    {\int\!#1\,}% script
    {\int\!#1\,}% scriptscript
}

% \mltint[3] -> \int\int\int with better spacing
\newcounter{multintctr}
\newcommand{\mltint}[1][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \int}

\newcommand{\mltintdx}[2][1]{%
  \setcounter{multintctr}{1}%
  \whiledo{\value{multintctr}<#1}{%
    \int\!\!\!\!%
    \stepcounter{multintctr}%
  }%
  \intdx[#2]}

% more latex log-like functions
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
%\newcommand{\argmax}{\mathop{\mathbox{argmax}}}
%\newcommand{\argmin}{\mathop{\mathbox{argmin}}}
\newcommand{\erfc}{\mathop{\mathbox{erfc}}}

\newcommand{\map}{\ensuremath{{\mathbox{\textsf{MP}}}}}
\newcommand{\ml}{\ensuremath{{\mathbox{\textsf{ML}}}}}
\newcommand{\new}{\ensuremath{{\mathbox{\textsf{new}}}}}

% number sets
% \newcommand{\reals}{\mathsf{I\!R}}
\newcommand{\complexes}{\mathbb{C}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\integers}{\mathbb{Z}}
\newcommand{\naturalss}{\mathbb{N}}

% hypotheses
\newcommand{\model}[1]{\ensuremath{\mathcal{M}_{#1}}}

% abbrevs for some greeks
\newcommand{\eps}{\ensuremath{\epsilon}}
\newcommand{\ohm}{\ensuremath{\Omega}}

% ion types
\newcommand{\sodium}{\ensuremath{\mathbox{Na}^+}}
\newcommand{\potassium}{\ensuremath{\mathbox{K}^+}}
\newcommand{\calcium}{\ensuremath{\mathbox{Ca}^{++}}}

% HMM nulls and collisions
%\newcommand{\nll}{\ensuremath{\mathbox{\o}}}
\newcommand{\cll}{\ensuremath{\mathchoice{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
{c\!\!{\scriptscriptstyle /}}%
}}
\newcommand{\Null}[2]{\ensuremath{\mathbox{\O}}_{#1,#2}}

\newcommand{\sumrows}[1]{\ensuremath{\left\langle{#1}\right\rangle}}
\newcommand{\sumcols}[1]{\ensuremath{\overline{\underline{#1}}}}

% equal by definition
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}}

% llllllllllong arrows
\def\llongrightarrow{-\mkern-8.5mu\longrightarrow}
\def\lllongrightarrow{-\mkern-3mu-\mkern-8.5mu\longrightarrow}




% accents

% from symbols-a4.pdf; optional arg permits shortening to prevent
% adjacent bars running together
\newcommand{\widebar}[2][3]{{}\mkern#1mu\overline{\mkern-#1mu#2}}

% struts useful for artificially enlarging latex \left\right
% constructs: e.g. \angles{\Bigstrut x}
% \strut ~= \big
% \Bigstrut ~= \Big
% \biggstrut ~= \bigg
%
%  Turns out we can just use \Big. and similar to do this.  Which
%  means it works with exscale.sty (which rescales the \big defs to
%  match the fontsize) too.
\def\bigstrut{\big.}
\def\Bigstrut{\Big.}
\def\biggstrut{\bigg.}
\def\Biggstrut{\Bigg.}

%% overrideable left-right delimeters
% \lr(){foo} -> \left(foo\right)
% \lr[]{foo} -> \left[foo\right]
% \lr[\big](){foo} -> \big({foo}\big)
% \lr[][]{foo} -> \left[{foo}\right]  -- double [] to avoid delims begin processed as (empty) opt
% \lr\{\}{a \lrmid | b } will re-scale the `|' appropriately
% \lr{}{}{foo} -> foo -- this is useful to clobber delims when lr is called from other macros
% this version should nest correctly.  
\newcommand\lr[4][]{%
  \ifthenelse{\equal{#2{}}{{}} \and \equal{#3{}}{{}}}%
             {#4}%
             {\ifthenelse{\equal{#1{}}{{}}}%
               {{\left#2\def\lrmid{\middle}#4\right#3}}% extra {}s to limit scope of def
               {{#1#2\def\lrmid{#1}#4#1#3}}% extra {}s to limit scope of def
             }%
}
% \makeatletter
% \newcommand\lr[4][]{%
%   \ifthenelse{\equal{#1{}}{{}}}%
%              {\def\@lrcontent{#4}%
%                \mathopen{\left#2\vphantom\def\lrmid{\middle}#4\right#3}}% extra {}s to limit scope of def
%              {{#1#2\def\lrmid{#1}#4#1#3}}% extra {}s to limit scope of def
% }
% \makeatother

% % old version -- use \lrset( \lrset) in place of \left( right).  Cannot be nested!!
% \newboolean{inlr}
% \newboolean{midlr}
% \setboolean{inlr}{false}
% \newcommand\newlr{\setboolean{inlr}{false}}
% 
% \newcommand\lrset[1]{%
%   \ifthenelse{\boolean{inlr}}%
%     {\ifthenelse{\boolean{midlr}}%
%       {\middle#1\setboolean{inlr}{true}}
%       {\right#1}}%
%     {\left#1\setboolean{inlr}{true}}}%
% \newcommand\lrmid{%
%   \ifthenelse{\boolean{inlr}}%
%     {\setboolean{midlr}{true}}
%     {}}%




